Model Checking Gene Regulatory Networks

The behaviour of gene regulatory networks (GRNs) is typically analysed using simulation-based statistical testing-like methods. In this paper, we demonstrate that we can replace this approach by a formal verification-like method that gives higher assurance and scalability. We focus on Wagner weighted GRN model with varying weights, which is used in evolutionary biology. In the model, weight parameters represent the gene interaction strength that may change due to genetic mutations. For a property of interest, we synthesise the constraints over the parameter space that represent the set of GRNs satisfying the property. We experimentally show that our parameter synthesis procedure computes the mutational robustness of GRNs -an important problem of interest in evolutionary biology- more efficiently than the classical simulation method. We specify the property in linear temporal logics. We employ symbolic bounded model checking and SMT solving to compute the space of GRNs that satisfy the property, which amounts to synthesizing a set of linear constraints on the weights.

==> Makefile <==
# Makefile for papers 
MAIN = main
.PHONY: clean open spell $(MAIN).pdf

all: $(MAIN).pdf

$(MAIN).pdf: *.tex $(MAIN).bbl
	pdflatex $(MAIN)
	pdflatex $(MAIN)
	killall -s HUP -q mupdf

$(MAIN).bbl: biblio.bib $(MAIN).tex
	pdflatex $(MAIN)
	bibtex $(MAIN)

spell:
	aspell -t -c $(MAIN).tex

zip:
	zip -r main.zip *

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
latex:
	@echo latex $(MAIN).tex </dev/null
	@if latex $(MAIN).tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch $(MAIN).dvi; exit $$stat; \
	fi 
	bibtex $(MAIN) || true
	@echo latex $(MAIN).tex </dev/null
	@while grep "Rerun to get cross" $(MAIN).log; do \
		echo latex $(MAIN).tex </dev/null; \
		if latex $(MAIN).tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch $(MAIN).dvi; exit $$stat; \
		fi; \
	done
	dvips -e 0 -t letter -P pdf -o $(MAIN).ps $(MAIN).dvi ;

clean:
	rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).log $(MAIN).out $(MAIN).ps $(MAIN).pdf $(MAIN).dvi $(MAIN).blg *.bak *.auto *.log *~ */*~ */texput.log




==> fig/fig-bi-stable-robust.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\textwidth]{imgs/picAB_labelled.pdf}
\caption{
\tanja{try to change the figure.. can't open the original file}
Robustness of cross-inhibition example.
%
(a) The set of constraints over parameters which affect the dynamics of $\grnU$
and $\grnR$.
%
(b) A part of the parametrized labeled transition system for $\grn$:
%
each transition is labeled by a set of constraints which render it feasible.
%
The commas between the constraints denote logical conjunctions.
%
The formula $\bar{\prop}$ denotes the negation of $\prop$.
%
The solid lines are transitions which will occur in a system with bistability.
%
The dotted lines represent the traces which do not exhibit the phenotype.
%
(c) For fixed values $\weight_{AB}=\weight_{BA} = \weight_{BB}=0.3$, $\threshA=\threshB=0.6$, and
varying values of $\inA$ and $\inB$, we plot the regions of parameter
space which preserve the phenotype.
The $\alpha_0\wedge\alpha_1\wedge\beta_0\wedge\beta_1$ and
$\alpha_0\wedge\alpha_1\wedge\beta_0\wedge\beta_1'$ regions
correspond to $\grnU$ and $\grnR$ respectively.
}
\label{fig:abL}
\end{figure}

%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/fig-bi-stable.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{imgs/picAB_tacas_.pdf}
\caption{Gene interaction schemes for cross-inhibition between genes $A$ and $B$.
}
\label{fig:ab}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/fig-examples.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{imgs/GRNmotifs.pdf}
\caption{
The constraints for GRN motifs for $l=3$, $tB=0.5$ and $t_C=0.9$.
a) GRN landscapes $\grnP_1$ and $\grnP_1'$. The thick solid line denotes the region of weights there the property $\prop_1$ holds, and the dotted line represent the region where $\prop_1'$ holds.
b) The region of weights where GRN landscape $\grnP_2$ satisfies $\prop_2$.}
% and $\grnP_2'$. The region where $\prop_2$ holds is equivalent for both landscapes.}
\label{fig:motifs}
\end{figure}

%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 




==> fig/fig-examplesMotifs.tex <==
%%\label{sec:bio-mutation-model}
%\begin{figure}
%%\begin{centering}
%\includegraphics[scale=0.25]{imgs/GRNmotifs.pdf}
%\caption{Genetic motifs introduced in \secref{moreExamples}, graphical illustration of the regions satisfying the formulae. }
%\label{fig:a1}
%\end{figure}


%\label{sec:bio-mutation-model}
\begin{figure}
%\begin{centering}
\includegraphics[scale=0.25]{imgs/evolutionaryModels.pdf}
\caption{
Illustration of the evolutionary process for the GRN motif example introduced in 
\figref{fig:motifs}a), for parameter values $\weight_A=\weight_B=0.9$, $\thresh_A=0.5$, $\thresh_B=0.9$.
%\secref{moreExamples}:
a) transition probabilities from one GRN to another. 
Each GRN is represented by listing the number of mutations which occur at each of the genes.
b) In the mutation model with selection, the robustness is the probability that individual will survive in the next generation; The shaded region represents the surviving configurations. The marked transitions are the ones which lead to cell death.}
\label{fig:evolGRN}
\end{figure}

==> fig/fig-grns.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{imgs/ABCnew.pdf}
\caption{
Feed-forward loop: % $w_A=w_B=w_C=1$, $t_B=0.5$, $t_C=0.9$. %, $i_B=i_C=0.95$.
type I coherent ($\grn_1$), % and after removing gene $B$ ($\grn_1'$), and %: Sign-sensitive delay.
type I incoherent ($\grn_2$), and
the repressilator (type IV incoherent, $\grn_3$).%: Puls generator.
}
\label{fig:motifs}
\end{figure}

==> fig/fig-mi.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{imgs/mi.pdf}
\caption{
..
}
\label{fig:motifs}
\end{figure}

==> fig/fig-misu.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\textwidth]{imgs/img_example_misu.pdf}
\caption{Gene interaction schemes for cross-inhibition between genes $A$ and $B$.
}
\label{fig:ab}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/fig-mutation.tex <==
\begin{figure}
\centering  
  \def\offgencolor{black!10}
  \newcommand{\zerozero}{\tiny$\{A{\color{\offgencolor}{,B,C}}\}$}
  \newcommand{\zeroone}{\tiny$\{A,{\color{\offgencolor}{B,}}C\}$}
  \newcommand{\onezero}{\tiny$\{A,B{\color{\offgencolor}{,C}}\}$}
  \newcommand{\oneone}{\tiny$\{A,B,C\}$}

  \newcommand{\distance}{1.8}

  \def\reallybrokenstt{
    \begin{tikzpicture}
      \node[state] (00) at (0,0) {\zerozero};
      \node[state] (01) at (\distance,0) {\zeroone};
      \node[state] (10) at (0,-\distance) {\onezero};
      \node[state] (11) at (\distance,-\distance) {\oneone};
      
      \path[->] (00) edge [loop above] (00)
                (01) edge (00)
                (10) edge (00)
                (11) edge (00)
                (11) edge [draw=none,loop below] (11);%placeholder
    \end{tikzpicture}
  }

  \def\brokenstt{
    \begin{tikzpicture}
      \node[state] (00) at (0,0) {\zerozero};
      \node[state] (01) at (\distance,0) {\zeroone};
      \node[state] (10) at (0,-\distance) {\onezero};
      \node[state] (11) at (\distance,-\distance) {\oneone};
      
      \path[->] (00) edge [loop above,draw=none] (00)%placeholder
                (00) edge (10)
                (01) edge (10)
                (10) edge [loop below] (10)
                (11) edge (10);
    \end{tikzpicture}
  }

  \def\goodstt{
     \begin{tikzpicture}
       \node[state] (00) at (0,0) {\zerozero};
       \node[state] (01) at (\distance,0) {\zeroone};
       \node[state] (10) at (0,-\distance) {\onezero};
       \node[state] (11) at (\distance,-\distance) {\oneone};
       
       \path[->] (00) edge [loop above,draw=none] (00)%placeholder
                 (00) edge (10)
                 (01) edge (10)
                 (10) edge (11)
                 (11) edge [loop below] (11);
     \end{tikzpicture}
  }

  \def\labelshift{5mm}
  \begin{tikzpicture}
    \node (reallybroken) {\reallybrokenstt};
    \node (broken) [right =1cm of reallybroken] {\brokenstt};
    \node (good) [right =1cm of broken] {\goodstt};
  
    \node [below=-\labelshift of reallybroken] {(a)};
    \node [below=-\labelshift of broken] {(b)};
    \node [below=-\labelshift of good] {(c)};
  \end{tikzpicture}
  \caption{Transition systems induced by mutations on GRN of
\Fig{fig:ffl_grn}a. 
% \tocolleagues{In this picture I am making the assumption that A is always expressed. Actually without resolving the ambiguity on the semantics of the canalization model we cannot sketch the graphs. With double threshold we could have non deterministic state transition graphs.}
}
  \label{fig:mut}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/fig-weighted-grn-AB.tex <==
\begin{figure}
  \centering
  \def\goodffl{
    \begin{tikzpicture}
      \node [gen] (B) at (2,0) {\tiny$\thresh(B)$, $\weight(B)$};
      \node [gen] (A) at (0,0) {\tiny$\thresh(A)$, $\weight(A)$}
      edge [rep, bend right=30] node [auto,swap] {} (B); %\tiny$\weightvar{A} = \fracwb$} (B);
      edge [rep, bend left=30] node [auto] {} (A); %\tiny$\weightvar{B} = \fracwb$} (A);
     % \node [gen] (A) [above of=B,xshift=1cm, yshift=0.5cm] {A}
      %edge [act, bend left=30] node [auto] {\tiny$\weightvar{A} = \fracwa$} (C)
      %edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{A} = \fracwa$} (B);
      
      \begin{scope}[on background layer]
        \fill[green!50] (B.west) arc (0:180:-5mm)--cycle;
        \fill[black!20] (B.east) arc (0:180:5mm)--cycle;
      \end{scope}
    \end{tikzpicture}
  }

  \def\badffl{
    \begin{tikzpicture}
      \node [gen,fill opacity=0,text opacity=1] (B) at (2,0) {\tiny$\thresh(B)=\fractc$};
      \node [gen] (A) at (0,0) {\tiny$\thresh(A)=\fractb$}
      edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{A} = \fracmutwb$} (B);
      %\node [gen] (A) [above of=B,xshift=1cm, yshift=0.5cm] {A}
      %edge [act, bend left=30] node [auto] {\tiny$\weightvar{A} = \fracwa$} (C)
      %edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{A} = \fracwa$} (B);
      
      \begin{scope}[on background layer]
        \fill[green!50] (A.west) arc (0:180:-5mm)--cycle;
        \fill[black!20] (A.east) arc (0:180:5mm)--cycle;
      \end{scope}
    \end{tikzpicture}
  }

  \def\labelshift{0mm}
  \begin{tikzpicture}
    \node (good) {\goodffl};
    \node (bad) [right =1cm of good] {\badffl};
    
    \node [below=-\labelshift of good] {(a)};
    \node [below=-\labelshift of bad] {(b)};
  \end{tikzpicture}

  \caption{Cross-inhibition network}
\label{fig:ffl_grn}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End: 


==> fig/fig-weighted-grn.tex <==
\begin{figure}
  \centering
  \def\goodffl{
    \begin{tikzpicture}
      \node [gen] (C) at (2,0) {\tiny$\thresh(C)=\fractc$};
      \node [gen] (B) at (0,0) {\tiny$\thresh(B)=\fractb$}
      edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{B} = \fracwb$} (C);
      \node [gen] (A) [above of=B,xshift=1cm, yshift=0.5cm] {A}
      edge [act, bend left=30] node [auto] {\tiny$\weightvar{A} = \fracwa$} (C)
      edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{A} = \fracwa$} (B);
      
      \begin{scope}[on background layer]
        \fill[green!50] (A.west) arc (0:180:-5mm)--cycle;
        \fill[black!20] (A.east) arc (0:180:5mm)--cycle;
      \end{scope}
    \end{tikzpicture}
  }

  \def\badffl{
    \begin{tikzpicture}
      \node [gen,fill opacity=0,text opacity=1] (C) at (2,0) {\tiny$\thresh(C)=\fractc$};
      \node [gen] (B) at (0,0) {\tiny$\thresh(B)=\fractb$}
      edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{B} = \fracmutwb$} (C);
      \node [gen] (A) [above of=B,xshift=1cm, yshift=0.5cm] {A}
      edge [act, bend left=30] node [auto] {\tiny$\weightvar{A} = \fracwa$} (C)
      edge [act, bend right=30] node [auto,swap] {\tiny$\weightvar{A} = \fracwa$} (B);
      
      \begin{scope}[on background layer]
        \fill[green!50] (A.west) arc (0:180:-5mm)--cycle;
        \fill[black!20] (A.east) arc (0:180:5mm)--cycle;
      \end{scope}
    \end{tikzpicture}
  }

  \def\labelshift{0mm}
  \begin{tikzpicture}
    \node (good) {\goodffl};
    \node (bad) [right =1cm of good] {\badffl};
    
    \node [below=-\labelshift of good] {(a)};
    \node [below=-\labelshift of bad] {(b)};
  \end{tikzpicture}

  \caption{A feed-forward loop GRN}
\label{fig:ffl_grn}
\end{figure}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: main
%%% End: 


==> fig/tab-benchmark-appr.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{ccccc}
&\multicolumn{2}{c}{\textsc{Approximate computation of robustness}}\\
\toprule
GRN & \multicolumn{1}{c}{Value} &  \multicolumn{2}{c}{Total time} \\
& \textsc{Symbolic or Explicit} & \textsc{Symbolic} & \textsc{Explicit}  \\
\midrule
%epigenetic switch, $l=1$ & $0.99707$ & $0.99707$  & $0.01$ & $0$ \\
%mutual inhibition, $l=1$ &  $0.003906$ & $0.003906$ &  $0.00990099$ & $0$\\
epigenetic switch ($l=5$) & $0.9999419\pm 2.51E-05$ & $0.9214851$ & $1.14495$\\
mutual inhibition ($l=5$) &  $9.29E-05\pm 2.7E-0.5$ &  $1.069406$ & $1.814356$\\
\bottomrule
\end{tabular}
\caption{
%
The comparison of the symbolic and explicit approach when the robustness is computed by approximately, that is, by sampling the GRN's from the landscape.
%
We evaluate robustness from $100$ sets of $10^5$ sampled points.
}
\label{tab:benchmark}
\end{figure}


%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/tab-benchmark-full.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{ll|c|cc|cc|c}
\toprule
\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Simulation} & \multicolumn{2}{c}{Model checking}  & \multicolumn{2}{c}{Ammortization} & Impr.\\
\multicolumn{1}{c}{name} & \multicolumn{1}{c}{slope} & \multicolumn{1}{c}{intercept} & \multicolumn{1}{c}{slope} & \multicolumn{1}{c}{\#mutants} & \multicolumn{1}{c}{$\sigma^2 / \mu$} & $dB$\\
\midrule
%%\texttt{am} & 2 + 2 & $\sci{2.27}{-2}$ & $\bf\sci{3.62}{-7}$ & $\sci{4.05}{-6}$ \\
\texttt{mi}    & $\sci{1.32}{-5}$ & $\sci{2.78}{-2}$ & $\bf\sci{8.56}{-6}$ & $\sci{5.6}{3}$ &  & $+1.88$\\
\texttt{misa}  & $\sci{1.77}{-5}$ & $\sci{1.36}{-2}$ & $\bf\sci{8.83}{-6}$ & $\sci{1.53}{3}$ & $\sci{9.08}{-5}$ & $+3.02$\\
\texttt{qi}  & $\sci{2.67}{-5}$ & $\sci{2.94}{-1}$ & $\sci{3.25}{-5}$ & -- & -- & $-0.85$\\
\texttt{cc}  & $\sci{2.12}{-5}$ & $\sci{2.51}{-1}$ & $\bf\sci{1.35}{-5}$ & $\sci{3.29}{4}$ & $\sci{1.45}{-5}$ & $+1.96$\\
\texttt{ncc} & $\sci{3.63}{-5}$ & $\sci{7.03}{+1}$ & $\sci{6.36}{-5}$ & -- & -- & $-2.44$\\
\midrule
\texttt{osc3} & $\sci{1.27}{-5}$ & $\sci{3.13}{-2}$ & $\bf\sci{6.71}{-6}$ & $\sci{5.22}{3}$ & $\sci{4.44}{-4}$ & $+2.77$ \\
\texttt{osc5}  & $\sci{3.50}{-5}$ & $\sci{5.80}{-1}$ & $\bf\sci{2.16}{-5}$ & $\sci{4.31}{4}$ & -- & $+2.10$\\
\texttt{osc7}  & $\sci{5.30}{-5}$ & $\sci{1.67}{+1}$ & $\bf\sci{1.72}{-5}$ & $\sci{4.71}{5}$ & -- & $+4.89$\\
\bottomrule
\end{tabular}
\caption{
Linear regression of time evaluation w.r.t. number of mutants, i.e., \newline \emph{time} = \emph{slope} $\cdot$ \#\emph{mutants} + \emph{intercept}.
}
\label{tab:time}
\end{figure}

%\begin{figure}[t]
%\centering
%\begin{tabular}{ccccc}
%&\multicolumn{1}{c}{\textsc{Exact computation of robustness}}\\
%\toprule
%GRN & \multicolumn{1}{c}{Value} &  \multicolumn{2}{c}{Toatl time} \\
%& \textsc{Symbolic} or {Explicit} & \textsc{Symbolic} & \textsc{Explicit}  \\
%\midrule
%%epigenetic switch, $l=1$ & $0.99707$ & $0.99707$  & $0.01$ & $0$ \\
%%mutual inhibition, $l=1$ &  $0.003906$ & $0.003906$ &  $0.00990099$ & $0$\\
%epigenetic switch ($l=5$) & $0.999945$  & $0.2067327$ & $0.479901$ \\
%mutual inhibition ($l=5$) &  $9.5E-05$  &  $0.04$ & $0.1509901$\\
%\bottomrule
%\end{tabular}
%\caption{
%%
%The comparison of the symbolic and explicit approach when the robustness is computed exactly, that is, via enumerating all weights from the \GRNlandscape. 
%}
%\label{tab:benchmark}
%\end{figure}


%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> fig/tab-benchmark.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{|c|c|c|c|c|}
\toprule
{Model} &{\#Genes} & {\# Edges}  & {Property} & Size of GRN space \\
%\multicolumn{1}{c}{name} & \multicolumn{1}{c}{size} & \multicolumn{1}{c}{slope} & \multicolumn{1}{c}{intercept} & \multicolumn{1}{c}{slope} & \multicolumn{1}{c}{\#mutants} & \multicolumn{1}{c}{$\sigma^2 / \mu$} & $dB$\\
\midrule
%%\texttt{am} & 2 + 2 & $\sci{2.27}{-2}$ & $\bf\sci{3.62}{-7}$ & $\sci{4.05}{-6}$ \\
mutual inhibition -- \texttt{mi} & 2 & 2 & bistability & $4225$  \\
mutual inhibition -- \texttt{misa} & 2 & 4& bistability &  $105625$\\
quad inhibition -- \texttt{qi} & 4 & 8 & bistability &  $\approx10^9$\\
cell cycle switch -- \texttt{cc} & 5 & 6 & bistability &  $\approx 10^{10}$\\
cell cycle switch -- \texttt{ncc} & 6 & 12 & bistability &  $\approx10^{18}$\\
\midrule
oscillator -- \texttt{osc3} & 3 & 3 & oscillation &  $274625$ \\
oscillator -- \texttt{osc5} & 5 & 5 & oscillation &  $\approx10^9$\\
oscillator -- \texttt{osc7} & 7 & 7 & oscillation &  $\approx10^{12}$\\
\bottomrule
\end{tabular}
\caption{
The characteristics of GRNs used to benchmark the robustness computation.
%
%the length of binding site for the input gene set to twelve, and other equal to four.
}
\label{tab:characteristics}
\end{figure}

%\begin{figure}[t]
%\centering
%\begin{tabular}{ccccc}
%&\multicolumn{1}{c}{\textsc{Exact computation of robustness}}\\
%\toprule
%GRN & \multicolumn{1}{c}{Value} &  \multicolumn{2}{c}{Toatl time} \\
%& \textsc{Symbolic} or {Explicit} & \textsc{Symbolic} & \textsc{Explicit}  \\
%\midrule
%%epigenetic switch, $l=1$ & $0.99707$ & $0.99707$  & $0.01$ & $0$ \\
%%mutual inhibition, $l=1$ &  $0.003906$ & $0.003906$ &  $0.00990099$ & $0$\\
%epigenetic switch ($l=5$) & $0.999945$  & $0.2067327$ & $0.479901$ \\
%mutual inhibition ($l=5$) &  $9.5E-05$  &  $0.04$ & $0.1509901$\\
%\bottomrule
%\end{tabular}
%\caption{
%%
%The comparison of the symbolic and explicit approach when the robustness is computed exactly, that is, via enumerating all weights from the \GRNlandscape. 
%}
%\label{tab:benchmark}
%\end{figure}


%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> fig/tab-rob.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{lllllllll}
$\#$ genes & $3$ & $4$ & $5$ & $6$ & $7-9$ \\ %& $8$ & $9$ & $10$ \\
\hline
%robustness & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & $10$ \\
max. time & $\leq 0.01$ & $0.02$ & $0.4$ & $15.13$ & T/out\\%& $7$ \\%& $8$ & $9$ & $10$ \\
%max. time ($l=5$) & $0.05$ & $5.9$ & $0.4$ & $29.96$ & $7$ & $8$ & $9$ & $10$ \\
\hline
%0sec & 
%\topple
%\#$G$ & \multicolumn{3}{c|}{Our method} & \multicolumn{2}{c}{Simulation} \\
%& \textsc{Gen} & \textsc{Eval} & \textsc{Compl.} & \textsc{Sim} & \textsc{Compl.}  \\
%\midrule
%3 & 0.07s & 1.29s & 100\% & 3.01s & 100\% \\
%4 & 0.13s & 1.68s & 100\% & 5.35s & 100\% \\
%5 & 0.23s & 2.09s & 100\% & 7.28s & 100\% \\
%6 & 0.67s & 2.48s & 100\% & 9.19s & 100\%  \\
%7 & 2.52s & 2.87s & 100\% & 10.58s & 100\% \\
%8 & 7.91s & 3.19s & 99\% & 12.66s  & 100\% \\
%9 & 29.00s & 3.59s & 91\% & 12.65s & 100\% \\
%10 & 40.87s & 3.95s & 71\% & 14.92s & 100\% \\
%\bottomrule
\end{tabular}
\caption{
The maximum computation time among ten randomly generated networks with a given number of genes and length of binding site $l=3$ for all genes. 
}
\label{tab:rob}
\end{figure}


%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig/table-grns.tex <==

\begin{table}[t]
\centering
%\begin{tabular}{c| c c c c c}
%\hline\hline
%$(p,l,\thresh_B,\thresh_C)$ & $(0.5,4,0.1,0.9)$ & 
%$(0.5,4,0.9,0.1)$& $(0.5,19,0.5,0.5)$ &  $(0.75,19,0.5,0.5)$\\ [0.5ex] 
%\hline
%$\grn_1$ wrt $\prop_1$ & 0.574 & 
%0.059 & 
%0.25 & 0.009\\
%$\grn_1'$ wrt $\prop_1$ 
% & 0.0625 
%& 0.9375 & 0.5 & 0.991\\
%%$\prop_1(\grn_2)$ & ... \\
%$\grn_2$ wrt $\prop_2$ & 0.059 %&  0.191 
%& 0.004 & 0.499 & 0.991\\ [1ex]
%\hline
%\end{tabular}
\begin{tabular}{c| c c c }
\hline\hline
$p$ & $0.25$ & $0.5$ & $0.75$  \\ [0.5ex] 
\hline
$\grn_1$ wrt $\prop_1$ & 0.059 & 0.25 & 0.009\\
$\grn_1'$ wrt $\prop_1$ & 0.9375 & 0.5 & 0.991\\
$\grn_2$ wrt $\prop_2$ & 0.004 & 0.499 & 0.991\\ [1ex]
\hline
\end{tabular} 
\caption{Robustness of GRN motifs. $p$ denotes the probability of a single-point mutation. 
All experiments were done for promoter length $l=2$, $w_A=w_B=w_C=0.5$, $t_A =t_B=t_C=0.5$. 
%$(p,l,t_B,t_C)$ denote respectively the probability of a single mutation, length of the promoter region, threshold for activation of gene $B$ and threshold for activation of gene $C$.
}
\label{table:motifs}
\end{table}

==> tex_parts/LTL-discussion.tex <==

\section{Discussion over LTL}
In this section we will introduce the concept of function of a GRN. 
In any organism the function of the gene regulatory system is
to transcribe subsequences of DNA into mRNA, that will be than
translated in proteins. Then the produced proteins will follow
different pathways, included the one of participating in the gene
regulation themselves. Summarizing, the main function is to express
genes following determined behaviors or patterns with respect to time. 

A simple pattern of gene regulation is the continuous expression,
meaning that a certain gene is required to remain expressed during all
the live of the system. 
Continuous unexpression, under certain conditions like signals or
initial conditions, could be necessary for the correct behavior of the
cell. Causality among states, meaning that gene expression must follow
a precise order of activation or repression of other genes, in order
to avoid misbehavior. 
The existence of attractors, which means that after some point a
certain condition must hold for life of the system, potentially with
multi-modal behavior. 
In case of multi-modal behavior the organism is required to show
determined expression patterns in alternation but infinitely often. 



==> tex_parts/bio-mutation-model.tex <==
\section{Mutation model}
\label{sec:bio-mutation-model}

%
%Gene activation %transcription process 
%is initiated when a transcription factor binds to the promoter region of gene $\gene$.
%%
%A mutation in the promoter region may affect the binding affinity to the transcription factor, and, consequently, that gene's activity; 
%%
%We assume here that the maximal activity of gene $\gene$, that is, $\weight(\gene)$, is achieved for a single sequence of nucleotides, %${\avec}$,
%and that it will linearly decrease with the number of mutated nucleotides (where `mutated' refers to being different to the sequence with maximal activity).
%%
%Moreover, assume $\prob$ to be a probability of a single point mutation occurring at any place of the genome.
%%
%Then, if $k$ out of $\length$ nucleotides in the promoter of gene $\gene$ are mutated,  
%the activity of $\gene$ becomes
%%$$\weight(k_i)(\gene_i):=
%$\weight(\gene)(1-\frac{k}{\length})$,
%with probability
%${\length\choose k}\prob^{k}(1-\prob)^{\length-k}$.

%The presented model rests on 
Each gene, a part of DNA which can be transcribed to a protein, is said to be \emph{active} when the protein encoded by $\gene$ is present in the cell.
The transcription process is initiated when a transcription factor binds to the promoter region of gene $\gene$.
A mutation in the promoter region may affect the binding affinity to the transcription factor, and, consequently, that gene's weight; 
We assume here that the maximal weight of gene $\gene$, that is, $\weight(\gene)$, is achieved for a single sequence of nucleotides, 
and that it will linearly decrease with the number of mutated nucleotides (where `mutated' refers to being different to the sequence with maximal weight).

A possible way of interpreting the mutation model used in this work is the following.
Imagine an experiment which starts with a population of cells, each having a promoter of gene $\gene$ in configuration $\avec_0=(\nuc_1,\ldots,\nuc_{\length})\in\{\ade,\tim,\cyt,\gua\}^{\length}$, that is some sequence of $\length$ nucleotides.
A mutation in the promoter region may affect the binding affinity to the transcription factor, and, consequently, the gene expression level; We assume that the maximal weight $\weight$ is achieved for a single sequence of nucleotides, ${\avec}$,
and that it will linearly decrease with the increasing number of mis-matching nucleotides.
This is clearly an oversimplification, since different mutations at the same site will have different effects in the binding energy and not all sites contribute in the same way to the total binding energy. However, it correlates with what is seen experimentally, where it is generally found that there is one ``preferred'' sequence, and mutations from that sequence decrease the total binding energy. As such, this assumption simplifies the modelling immensely without compromising too much of the biological detail.

We assume discrete generations and that mutations happen only during replication.
When the DNA is passed from the mother to the daughter cell, a nucleotide $\nuc_i$ can mutate to a different value with probability $p$, and, consequently, it can remain the same with probability $1-p$.  
Furthermore, we assume that the mutations occur only in the promoter region of genes and that the mutation events are independent within the whole genome, and independent of the history of mutations, as is typically assumed in biology.

%If we observe a cell after a large number of generation changes, it may have any possible promoter sequence from the set  $\{\ade,\tim,\cyt,\gua\}^{\length}$. 
%In fact, it can be shown that the probability to be in any particular sequence will eventually become stationary
%(because the underlying stochastic process is an irreducible, aperiodic discrete-time Markov chain \cite{norris97}).
%Let $\K\in\{0,\ldots,\length\}$ be a random variable such that $\K(\avec)=k$ denotes that $\avec$ differs from $\avec_0$ in exactly $k$ points.  
%Under all of the above assumptions, it is easy to see that the stationary distribution of $\K$ is indeed a binomial distribution
%$P(\K=k) = {\length\choose k}\prob^{k}(1-\prob)^{\length-k}$, and by independence assumption, $P(\mathbf{\K}=\kVec)$ is exactly the product on the right-hand side of Eq. \eqref{eq:prob}.


%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> tex_parts/linear-algebra-stuff.tex <==
%
%The evolution of a population of GRNs under mutations is represented
%by a random variable $\Wvec_n =
%(\Wrandom_n^1,\ldots,\Wrandom_n^d)\in\weightSet$, where $\Wrandom_n^i$
%indicates the weight of gene $i$ at generation $n$.
%%
%It is important to notice here that the processes $\Wrandom_n^i$ do
%not evolve in the same way as the mutations $\K^i_n$, and that a lemma
%similar to \lemref{lem:evolutionary} does not apply for the components
%$\Wrandom_n^i$.
%%
%This is because $\K^i_n$ describes the evolution of mutations where
%all possible mutation states can have a positive probability.
%% 
%In contrast, the weight configurations that failed to exhibit the
%expected phenotype are considered dead and will not have a positive
%probability.
%
%Let LTL property $\prop$ be the expected phenotype.
%%
%Let $f_{\prop}:\weightSet\to\{0,1\}$ be a partitioning of the set of
%weights depending on whether the property $\prop$ holds, that is:
%%
%\[
%f_{\prop}(\weight) \hbox{ iff } \grn(\weight)\models \prop.
%\]
%%
%Finally, the evolution of the GRNs with $\prop$-selection is a process $\{\Wvec_n\}$ over the state space $\weightSet$, where the initial probability is such that
%%
%\[
%\hbox{ if }f_{\prop}(\weight_{\kvec}) =0 \hbox{ then }P(\Wvec_0=\weight_{\kvec}) = 0,\] 
%%
%and the transient probabilities evolve according to the following recursive scheme:
%\begin{align}\label{eq:update} 
%%
%P(\Wvec_{n+1}=\weight_\kvec) =\frac{
%\displaystyle
%f_{\prop}(\weight_\kvec)
%\sum_{\weight_{\kvec'}\in\weightSet}P(\Wvec_n=\weight_{\kvec'})\Qmat(\kvec',\kvec)
%}
%{
%\displaystyle
%\sum_{\weight_{\kvec''}\in\weightSet}
%% \left(
%  \sum_{\weight_{\kvec'}\in\weightSet}
%  P(\Wvec_n=\weight_{\kvec'})
%  \Qmat(\kvec',\kvec'')
%% \right)
%}.
%\end{align}



\section{Evolution model}

\begin{proof}\rm(\lemref{lem:evolutionary})
It suffices to observe that $u$ represents the number of mutated nucleotides which remain mutated at time $(n+1)$, and $(j-u)$ is the number of unmated nucleotides which become mutated at time $(n+1)$.
The existence and convergence of the stationary trivially follows from that $\{\K_n\}$ is regular (irreducible and aperiodic).
Each process $\{X_n^i\}$ at a stationary behaves as a Bernoulli process, with probability of being mutated equal to $\beta=\lim_{n\to\infty} P(X_n^i=1)$, and a probability of remaining un-mutated $1-\beta$.
The claim follows as the sum of $l$ independent Bernoulli processes is binomially distributed.
The special case follows because matrix $\hat{P}^{id}$ has a unique stationary distribution $(0.25,0.75)$ (denoting by $a$ and $b$ its coordinates, we obtain equations $a(1-p)+b\frac{p}{3}=a$ and $ap+b(1-\frac{p}{3})=b$, which can be satisfied only if $a=\frac{b}{3}$).
\end{proof}

Remark that in a special case when $p_{00}=0.25$, 
%the matrix $P$ has rank one.
%Namely, if $p_{00}=p_{10}=0.25$, and $p_{01}=p_{11}=0.75$, then 
the transition matrix of the process $\{\K_t\}$ has the transition probabilities  
 \begin{align*}
P(K_{n+1}=j\mid K_n=i) & = p_{11}^{j}p_{00}^{l-j} \sum_{u=0}^i {i\choose u}{{l-i}\choose{j-u}} \\
 & = {l\choose j}0.75^{j}0.25^{l-j},
 \end{align*}
which do not depend on $i$.
%Then, trivially, the stationary distribution is the binomial distribution with single event probability $0.75$. 

\begin{proof} (\lemref{lem:conv})
The matrix ${\Qmat}$ due to the mutation model is obviously regular, because, from \eqref{eq:prob}, each two states have a non-zero transition probability.  
\end{proof}

\begin{proof} (\thmref{thm:stationary})
%Denote by $\tilde{\boldsymbol{\pi}}$, $\tilde{\Qmat}$ the restrictions of $\boldsymbol{\pi}$ and $\Qmat$ to the set of states ${\prop}(\weightSet)$, and
Denote by $\|\cdot\|$ the $1$-norm (sum of vector elements).
The definition of update of the probability distribution as shown in \dfnref{dfn:GRNL}, written in matrix notation amounts to:
\[
\tilde{\boldsymbol{\pi}}_{n+1}=\frac{\tilde{\boldsymbol{\pi}}_{n}\tilde{\Qmat}}{\|\tilde{\boldsymbol{\pi}}_{n}\tilde{\Qmat}\|}.
\]
The stationary distribution $\tilde{\boldsymbol{\pi}}$ satisfies $\tilde{\boldsymbol{\pi}}\|\tilde{\boldsymbol{\pi}} \tilde{\Qmat}\|=\tilde{\boldsymbol{\pi}} \tilde{\Qmat}$, and is therefore an eigenvector for $\tilde{\Qmat}$.
Since matrix $\tilde{\Qmat}$ is regular, there exist $k>0$ such that $\tilde{\Qmat}^k$ has all strictly positive entries. 
By the Perron-Frobenius theorem (\ref{thm:perron}), $\tilde{\Qmat}^k$ has a dominant eigenvalue with multiplicity one, which corresponds to a unique non-negative eigenvector space, scaled to $\tilde{\boldsymbol{\pi}}$.
The convergence follows from \thmref{thm:power}.

Finally, $\|\tilde{\boldsymbol{\pi}} \tilde{\Qmat}\|$ is the matrix form of \eqref{eq:rob} in \dfnref{dfn:robustness}, which proves the second part of the claim.  
\end{proof}


The following terminology and results can be found in any standard linear algebra textbook. % (e.g., see \cite{meyer2000matrix}).

\begin{definition} \rm
A matrix $M\in {\mathbf R}^{m\times n}$ is called positive (resp. non-negative), written $M>0$ (resp. $M\geq 0$), if all entries of $M$ are strictly positive (resp. non-negative).
\end{definition}

\begin{definition}\rm
A square matrix $M\in {\mathbf R}^{n\times n}$ is regular, if there exists $k>0$, such that $M^{k}\geq 0$.
\end{definition}

\begin{theorem} (Perron-Frobenious) \rm
Let $M$ be a square, positive matrix. %non-negative, regular matrix.
Then, 
\begin{enumerate}
\item $M$ has an eigenvalue $\hat{\lambda}\in {\mathbf R}_{>0}$, such that %, with positive left and right eigenvectors,
 for all other eigenvalues $\lambda$, we have $|\lambda|<\hat{\lambda}$,
  \item the right- and left- eigenvectors associated to eigenvalue $\hat{\lambda}$ are the only eigenvectors with all real, positive entries.
 %,and all other eigenvec
\item the eigenvalue $\hat{\lambda}$ has multiplicity one.
\end{enumerate}
\label{thm:perron}
\end{theorem}
%\clearpage
%\input{correct}

\begin{proof} (Sketch.)\rm
We only show the proof for (1). If $M$ has a spectral radius $\rho(M)$, then $M'=\frac{M}{\rho(M)}$ has an eigenvector on the unit circle, and all other eigenvalues of $M'$ are smaller or equal to $1$.
Assume $r=\rho(M')\neq 1$.
Then, there exists $m\in {\mathbb N}$, such that $Re(r^m)<0$. 
Notice that the matrix ${M'}^m-\epsilon I$ has all positive entries for some small enough $\epsilon>0$.
Moreover, by Gelfand's formula ($\lim_{k\to\infty} \|A^k\|^{1/k}=\rho(A)$ for any matrix norm $\|\cdot\|$), it follows that $\rho({M'}^m-\epsilon I)\leq \rho({M'}^m)\leq {\rho(M')}^m=1$.
On the other hand, since $({M'}^m-\epsilon I)v=(r^m-\epsilon)v$ for any vector $v$, it follows that $r^m-\epsilon$ is an eigenvalue for ${M'}^m-\epsilon I$, and consequently $\rho({M'}^m-\epsilon I)>\|r^m-\epsilon\|=1$. Contradiction.

Hence the spectral radius of $M$ is achieved for a positive real eigenvalue.
\end{proof}

\begin{theorem}\rm
Let $M$ be a square, non-negative, regular matrix.
If $v$ is the unit, left eigenvector for dominant eigenvalue $\hat{\lambda}$ with norm $1$, that is, $vM=\hat{\lambda}v$, then for all $v_0\in [0,1]^n$, such that $|v_0|=1$, $v_0$ has a non-zero component in the direction of the dominant eigenvector , and the sequence
 \[
 v_0, g(v_0), g^2(v_0), g^3(v_0),\ldots,
 \]
 where $g(w) :=  \frac{wM}{|wM|}$, 
 converges to $v$.
 \label{thm:power}
\end{theorem}

\begin{proof}(Sketch.)\rm
As $M$ is non-negative and regular, there exists $m>0$ such that $g^m(v_0)>0$. 
The convergence can be shown from the Jordan canonical form and by subsequently applying the power iteration approach.
Let $v_0$ be the initial distribution, and let $M=VJV^{-1}$ be the Jordan canonical form of $M$.
The vector $v_0$ can be written as a linear combination of the rows of $V^{-1}$ (generalized right eigenvectors):
$v_0=c_1v_1+\ldots+c_nv_n$,   
where $c_1\neq 0$ is non-negative eigenvector $v_1$ corresponding to the dominant eigenvalue.
%Then, %\tanja{ show that $c_1\neq 0$.}
%The rest of the proof can be found in \cite{}.
%Then,
%\begin{align*}
%v_0 M^k&=c_1\lambda_1^kv_1+\ldots+c_n\lambda_k^nv_n\\
%& = c_1\lambda_1^k(v_1+\ldots \frac{c_n}{c_1}\left(\frac{\lambda_n}{\lambda_1}\right)^k v_n),
%\end{align*}
%converges to $c_1\lambda_1^kv_1$ as $k\to\infty$. 
%%Since $M$ is a regular matrix, there exists $m>0$ such that all entries of $M^m$ are positive.
\end{proof}

\begin{lemma}\rm
A regular stochastic square matrix has a unique stationary distribution and it converges to it.
\end{lemma}

\begin{proof}\rm
Since all row sums are equal to $1$, the column vector of only ones is an eigenvector, and the corresponding eigenvalue is $1$. 
Hence, there exists a positive left eigenvector $\pi$ for eigenvalue $1$. 
Then, $\nu=\frac{\pi}{|\pi|}$ is a stationary distribution.
The proof of uniqueness and convergence follow as in the proof for \thmref{thm:perron} and \thmref{thm:power}. 
\end{proof}

%
%\begin{lemma}\rm
%The matrix $\Qmat$ derived for the evolution model is regular.
%% always aperiodic (each state has a non-zero self-loop), and the states with fitness $1$ which are reachable from the initial system form a strongly connected component.
%\end{lemma}
%The proof is trivial by construction of $\Qmat$ described in the mutation model (the transition between any two mutated states has a non-zero probability).

==> tex_parts/moreExamples.tex <==
\label{moreExamples}
\input{./fig/fig-grns}

%\noindent
%\subsection{Genetic network motifs}


\subsection{Examples}

We next illustrate how our robustness measure captures features of GRN motifs.
%We start with continuing the discussion of the motivating example, and continue with
We show three well-studied gene regulatory motifs with three genes, to which we express their known properties in LTL, and the resulting constraints.
{\em Genetic network motifs} are sub-networks which occur significantly more
frequently in gene regulatory networks than in a random graph with the
same statistical properties (that is, the number of nodes and graph density).
%
Various studies~\cite{milo2002network,shen2002network} have observed
that the GRNs $\grn_1$ and $\grn_2$ from~\figref{fig:motifs} are the
frequently occurring genetic network motifs, which are called {\em
coherent type-I} and {\em incoherent type-I} feed-forward loops
respectively.
%
The GRN $\grn_3$, also known as the \emph{repressilator}, was the model of a pioneering work in synthetic biology \cite{elowitz2000synthetic}, and it is known to provide oscillatory behaviour.
%
%We use our tool to compute the robustness for these gene regulatory
%motifs. 

\begin{example} \rm
$\grn_1$ is characteristic for having a ``sign-sensitive delay": when
the input signal is turned on, the output turns on with a delay, and
when the input signal is turned off, the output turns off quickly
afterwards.
%
The sign-sensitive delay can be encoded an LTL property 
\[\prop_1=(A\wedge \neg C \Rightarrow \ltlfinally C )
\wedge
(\neg{A}\wedge{C}\Rightarrow \ltlnext\neg{C}).% \hbox{ (noise rejection)}
\]
%
In words, when gene $a$ is on, the gene $c$ eventually turns on as well;
when gene $a$ is off, the gene $c$ immediately turns off.
%
However, deactivating $C$ is more difficult, %in $\grn_1$, 
because $B$ may still sustain $C$, even when $A$ is inactive.
%
The solution are the following constraints over parameters 
for $\grn_1$ %and $\grn_1'$.
\footnote{Simplified for presentation}: 
\begin{align*}
\grn_1 \models \prop_1  \hbox{ iff } \\
 \left[(\weight_A> \thresh_C)\vee (\weight_A>\thresh_B \wedge \weight_A+\weight_B>\thresh_C)\right] \wedge (\weight_B<\thresh_C).\\
%\grn_1' \models \prop_1 & \hbox{ iff } (\weight_A> \thresh_C)
\end{align*} 
The constraints are illustrated graphically in \figref{fig:evolGRN}.
\end{example}
% 
\begin{example}\rm
$\grn_2$ is characteristic for being a ``pulse generator"- when the
input signal is constantly on, the output signal will alternate
between states.
As a result, the constant input signal generates a pulse in the
output, which is described in LTL as follows:
\[\prop_2 =
 \neg{B} \Rightarrow \left[(A\wedge\neg{C}\Rightarrow \ltlnext C) \wedge
  (A\wedge C \Rightarrow \ltlfinally\neg{C})\right]. 
  \] 
%
In words, gene $c$ activates immediately after $a$, but gene $c$ will
also eventually deactivate under the presence of $a$.
%
The solutions are the following constraints over parameters 
for $\grn_2$.
\begin{align*}
\grn_2 \models \prop_{2} & \hbox{ iff } (\weight_A>\thresh_C) \wedge (\weight_A>\thresh_B \wedge \weight_A-\weight_B<\thresh_C).
\end{align*} 
\end{example}
%
\begin{example}\rm
\label{ex:oscilations}
The GRN $\grn_3$ generates oscillations: each gene should alternate its expression between `on' and `off' state:
%
\begin{align*}
\prop_{3} = \bigwedge_{v\in\{A,B,C\}}(v\wedge \Rightarrow \ltlfinally\neg{v})
\wedge 
(\neg{v}\wedge \Rightarrow \ltlfinally {v}).
\end{align*}
%In the model where each of the gene is activated, unless it is repressed by another gene, the 
%variant with gene states $\{-1,1\}$, the 
If all genes have constant inputs from the environment $i_A>0, i_B> 0, i_C>0$, the solutions are the constraints:
%
\begin{align*}
\grn_3 \models \prop_{3} & \hbox{ iff } (i_A>\thresh_A)\wedge(i_B>\thresh_B)\wedge(i_C>\thresh_C) \wedge\\
 &(i_B-\weight_A<\thresh_B) \wedge (i_C-\weight_B<\thresh_C) \wedge (i_A-\weight_C<\thresh_A).
\end{align*} 
\end{example}

\input{./fig/fig-examplesMotifs.tex}

%\subsection{Repressilator}


%
% As can be seen in \figref{fig:motifs}a, the satisfying regions of
% $\prop_{1}(\grn_1)$ and $\prop_{1}(\grn_1)$ can be disjoint.
%

%The interpretation of robustness value and its dependency %for different promoter region length and threshold values, and we compare it to 
% $\prop_1(\grn_2)$ \tableref{table:motifs}. 
% The constraints are as follows:

%the gene $c$ can turn on and off alternatively, whenever the input signal is always present.
%We also modify the network $\grn_2$ by again omitting the regulation via gene $B$ (`knocking-out' gene $B$), and adding self-inhibition to $C$ ($\grn_2'$ in \figref{fig:abc}b).


% \input{fig-examples.tex}


% It is clear that the network $\grn$ shows better robustness towards property 

%Upon varying the threshold values, we have observed that, for certain cases, $\grn_1'$ is more robust than $\grn_1$ for property $\prop_1$.
%This is because $\grn_1$ becomes more robust than $\grn_1'$ in cases when gene $A$ is not sufficient to activate $C$, but genes $A$ and $B$ can cooperatively activate $C$. 
%On the other hand, $\grn_1'$ is more robust than $\grn_1$ when 
%For many points in the mutation space, this is not the case, and, 
%
%for example, when threshold values for activating genes $B$ and gene $C$ are the same,
%the network $\grn$ is more robust to $\prop_1$, while when the threshold for activation of gene $B$ is  larger, the network $\grn$ is mor robust to $\prop_1$.
%In other words, motif can be found more robust than another
%\paragraph{Guiding the design of synthetic circuits}
%We show how our measure can be used to guide the robust design of synthetic circuits.
%
%We propose a simple memory circuit with two genes, where the design choice is the strength of the binding of transcription factors (TF's), incorporated in the model by a length of the promoter region and the activation threshold.
%
%We analyze the robustness of all possible three-gene network topologies prone to mutation. 
%Results show that the incoherent type-1 feed-forward loop (\cite{alon2007introduction}) most robustly exhibits the function of sign-sensitive delay.
%The coherent feed-forward loop with redundancy propagates the input signal more robustly than the linear network or the network where cooperation between input signals is necessary.

%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> tex_parts/running-example.tex <==
\section{Old Running example}

%\input{fig-feed-fwd-loop}
\input{./fig/fig-weighted-grn}
\begin{example}\label{ex:weights} 
%
In \Fig{fig:ffl_grn}, we present two GRNs consisting of three genes
$A$, $B$ and $C$,
which has similar network but different affinity functions.
GRNs with such network are called feed-forward loop~\cite{FFLCite}.
In the networks, the expression of $A$ induces the expression $B$ and
the expression of $A$ and $B$ induce the expression of $C$. 
Hence, the expression of $A$ eventually induces the expression of
$C$ that remains stable (as long as $A$ is expressed).
A feed-forward loop works correctly if expression of $A$ 
eventually induces stable expression of $C$.  
GRN in (a) shows a correctly behaving GRN where the binding
affinity of $A$ allows the activation of $B$ and the binding
affinities of $A$ and $B$ allow the activation of $C$. 
Note that $A$ and $B$ cooperatively activate $C$, meaning that both
are necessary. 
On the other hand, GRN in (b) does not display the correct behaviour
because 
$B$ does not sufficiently activate $C$, regardless of 
cooperative activation from $A$. 
Therefore, the expression of $A$ does not eventually induce the
activation of $C$. 
\end{example}

\ashu{@intro guys: Discuss historicity of this model }

\begin{example}\label{ex:prop} 
%
Consider the feed-forward loop GRN of \Ex{ex:weights} depicted in
\Fig{fig:ffl_grn}. 
The correct behaviour of that system can be summarized  by the
following sentence: \emph{as long as $A$ is expressed, after some
point $C$ will remain always expressed}. 
Such property is formally expressed in LTL as
\begin{align*}
\prop = \ltlglobally \genvar{A} \implies \ltlfinally \ltlglobally \genvar{C}~\text{.}
\end{align*} 
%
In other words, if $A$ is globally expressed, then eventually $C$ is
globally expressed. The GRN in \Fig{fig:ffl_grn}(a) satisfies the
property and the GRN in \Fig{fig:ffl_grn}(b) does not, as one can see
by their corresponding transition systems in \Fig{fig:mut}(c) and
\Fig{fig:mut}(b) (resp.).
\end{example}
\ashu{@intro guys: discuss we can express some cool stuff using this logic}


\begin{example}\label{ex:mut} 
%
Consider the feed-forward loop GRN discussed in the previous examples
and depicted in \Fig{fig:ffl_grn}. 
Consider the correctly behaving configuration, config. (a), as our
original system. 
Since mutations can only lower binding affinity, by assumption, the
space of feasible binding affinities is constrainted between $0$ and
$\fracwa$ both for gene $A$ and for gene $B$. We ignore gene $C$ since
it is not an active regulator. 
The thresholds of the regulated genes, genes $B$ and $C$ induce
constraints over the space of binding affinities. 
Sets of these constraints which satisfy the space of feasible binding
affinities represent sets of mutations that induce different
transition systems. 
The following table enumerates such sets:
\begin{center}
\begin{tabular}{l|l}
\toprule
transition system & Constraints\\
\midrule
(a) & $\{\weightvar{A} \le \fractb, \weightvar{A} \le \fractc, \weightvar{B} \le \fractc, \weightvar{A} + \weightvar{B} \le \fractc\}$ \\
(b) & $\{\weightvar{A} > \fractb, \weightvar{A} \le \fractc, \weightvar{B} \le \fractc, \weightvar{A} + \weightvar{B} \le \fractc\}$ \\
(c) & $\{\weightvar{A} > \fractb, \weightvar{A} \le \fractc, \weightvar{B} \le \fractc, \weightvar{A} + \weightvar{B} > \fractc\}$ \\
\bottomrule
\end{tabular}
\end{center} 
%
Each of the set induce the transition systems depicted in
\Fig{fig:mut} (with respective characters).
Structure (a) is induced by the mutations in which $A$ is too weak to stimulate $B$. 
Structure (b) is induced by the mutations in which $A$ is strong enough to stimulate $B$, but $A$ and $B$ together are too weak to stimulate $C$. 
Structure (c) is induced by mutations where $A$ can activate $B$ and $A$ and $B$ together can activate $C$. 
Structure (c) satisfies property $\prop$, while (a) and (b) do not.
\input{fig-mutation}
\end{example}

\begin{example}
Consider the original GRN where the length for the binding sites of $A$ and $B$ are $\length(A) = \length(B) = 5$. Mutations over the sequence of the binding sites induce dicrete points over the binding affinities space, where each point is a combination of the mutated affinities.
\input{fig-mutation-space}
\Fig{fig:mutspace} shows the dicrete lattice induced by mutations together with the boundaries of the constraints. The mutation $(\fracwa,\fracwb)$ corresponds to the original system (\Fig{fig:ffl_grn}a). 
It lays in the space of topology (a), which is the one that satisfy $\prop$. 
Mutations are reached by by flipping nucleatides one by one. 
If the mutated system still satisfies the property, further mutations can lead to a previous system or can lead to a new mutation. 
Conversely, if the new mutation crosses the boundary $\weightvar{A} + \weightvar{B} = \fractc$, the system \emph{dies} and no more mutations can happen. 
The mutation $(\fracwa,\fracmutwb)$ depicted in \Fig{fig:ffl_grn}b is case in which a is reached and then it dies.
\end{example}

The goal is to compute the cumulative probability mass of the
reachable mutations that satisfy a certain property. The probability
of a certain mutation is given by a binomial distribution with
probability of success $\frac{3}{4}$, i.e. the probability of
extracting a random nucleotide which different from the current one:
\begin{align*}
%% \prod_{\gen \in \gens} P\left(\frac{\length(\gen)\weightvar{\gen}}{\weight(\gen)} = B\left(\length(\gen), \frac{3}{4}\right)\right)
%% P(\mathcal{X} = \vec{\weightvar{}}) = \prod_{\gen \in \gens}  {\length(\gen) \choose \frac{\length(\gen)\weightvar{\gen}}{\weight(\gen)}} {\frac{3}{4}}^{\length(\gen)\left(\frac{\weightvar{\gen}}{\weight(\gen)}\right)}{\frac{1}{4}}^{\length(\gen)\left(1 - \frac{\weightvar{\gen}}{\weight(\gen)}\right)}
 %% \prod_{\gen \in \gens}  {\length(\gen) \choose \length(\gen)\frac{\weightvar{\gen}}{\weight(\gen)}} \left(\frac{3^{\weightvar{\gen}}}{3^{\weight(\gen)}\cdot 4}\right)^{\length(\gen)}
\mathbb{P}\bigg(\bigwedge_{\gen \in \gens} \weightvar{\gen} = \weight(\gen)\left(1 - \frac{k_\gen}{\length(\gen)}\right)\bigg) = \prod_{\gen \in \gens} {\length(\gen) \choose k_\gen} \left(\frac{3}{4}\right)^{k_\gen}\left(\frac{1}{4}\right)^{\length(\gen) - k_\gen}
\end{align*}
where $k_\gen \in \mathbb{N}$ is the number of flipped nucleotides on gene $\gen$.  

\begin{example}\ashu{@mirco: make sure well connected with rest of the text}
%
consider the property $\prop = \ltlglobally A \implies
\ltlfinally\ltlglobally C$. A counterexample for this property would
be a path $A$ is always expressed and the expression of $C$ is not an
attractor, namely its possible to reach infinitely ofter a state in
which $C$ is not expressed. Such witness in given by the formula
$\witness = \ltlglobally A \land \ltlglobally \ltlfinally \lnot C$. As
one can see from \Fig{fig:mut}, the bound $k = 2$ is enough to find
all witnesses. We show in the following a simplification of the
formula $\enc{\mutable, \witness}_k$:
\begin{align*} 
%
&\transenc{\mutable}{\genenc_{0}}{\genenc_{1}} \land
\transenc{\mutable}{\genenc_{0}}{\genenc_{1}} \land \\
(&\transenc{\mutable}{\genenc_{2}}{\genenc_{0}} \lor
\transenc{\mutable}{\genenc_{2}}{\genenc_{1}} \lor
\transenc{\mutable}{\genenc_{2}}{\genenc_{2}}) \land\\ (&A_0 \land A_1
\land A_2) \land (\lnot C_0 \lor \lnot C_1 \lor \lnot C_2)~\text{.}
\end{align*}  
\end{example}


\begin{example}
For example, the topology of \Fig{fig:mut4} is associated with the polyhedron is
\begin{align*}
\{-x_1 < -\frac{1}{2}, x_1 \le \frac{3}{4}, x_2 \le \frac{3}{4}, - x_1 - x_2 < -\frac{3}{4}\}
\end{align*} 


Let $A \in \{-1,0,1\}^d$ be the matrix of coefficients. We scale the
problem in order to move the mutations on the integer lattice. This is
given by the matrix $A' =
I_d\cdot(\frac{\weight(\gen_1)}{\length(\gen_1)}, \dots,
\frac{\weight(\gen_d)}{\length(\gen_d)})^\intercal$, where $\weight$
and $\length$ are weight and length functions as in
\Def{def:mutable}. The probability for a mutation on the lattice
$\mathbb{N}^d$ is given by a binomial distribution where the
components $k_1 \dots k_d$ give the number of flipped nucleotides
\begin{align*}
  \mathbb{P}(~\mathcal{K} = (k_1,\dots,k_d)~) = \prod_{i=1}^d {\length(\gen_i) \choose k_i} \frac{3}{4}^{k_1} \frac{1}{4}^{\length(\gen_i) - k_i}
\end{align*}
\end{example}



%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> tex_parts/variants.tex <==
%
In this section, 
we will discuss some variants of deterministic GRNs
that are also used in literature and their impact on computation of
robustness of GRNs.
%
Here we consider two variants. 
%
In the first variant the weights are assigned to the edges between the
genes instead of on the genes.
%
In the second variant, a gene state may take value from $\{-1,1\}$
instead of $\{0,1\}$.
%
Our method is applicable to each of the variants with slight modifications. 
%
%However, one variant may be amenable more conducive to 
%our analytical method then the others.
 


\subsection{Negative valued states}

So far, we have considered the more realistic model, in which gene
expression values are $0$ and $1$.
%
As stated before, Wagner's original formulation defined the range of
gene expression as a value between $-1$ and $1$.
% since this was sufficiently convenient for their analysis
%mostly interested in the evolution of \ashu{abstract properties??}.
%
While ~\dfnref{def:grn} transfers to this variant, the semantics is different.
%
A state $\state \colon \gens \to \{-1,1\}$ of a GRN
$\grn = (\gens, \acts, \reps, \weight, \thresh)$.

\begin{defn}[Transitions of a neg GRN]\label{def:grn-sem-neg}
$\trans \colon \states(\grn)
\to \states(\grn)$ is a deterministic transition function defined by
\begin{align*}
\trans(\state):= \lambda\gen'. % \mapsto 
sgn\hspace{-1ex}\left(
\quad
\sum_{\hspace{-8ex}\mathrlap{\{\gen \mid (\gen,\gen') \in \acts\}}} 
\state(\gen) \weight(\gen) ~-
\sum_{\hspace{-7ex}\mathrlap{\{ \gen \mid (\gen,\gen') \in \reps\}}}
\state(\gen) \weight(\gen)
 - \thresh(\gen')\right)\hspace{-1ex}\text{,}
\end{align*} 
where for $x>0$, $ sgn(x) =
\begin{cases}
  1  & \mbox{if } x > 0 \\
  -1 & \mbox{otherwise.}
\end{cases} $ 
\end{defn}

Notice that, in this model variant, the inhibited gene which represses 
another gene acts as an activator.
%
Subsequently the algorithm needs to be adapted in that %for our analysis algorithm, 
the definition of the parametrized transition system in Def~\ref{def:pts} 
changes.

\begin{defn}[Parametrized transition system]
\label{def:pts2}
%
For neg GRN $\grn = (G,\acts,\reps,\weight,\thresh)$ and 
rational parameters map $\wVar : G \to \allVars$, the {\em parametrized transition system}
$\transSys( \grn, \wVar )$ is a labelled transition system
$(\states(\grn), \states(\grn) \times \states(\grn), \transVar)$,
where
% \begin{itemize}
% \item 
  $\transVar : \states(\grn) \times \states(\grn) \to \polyhedra(\wVar)$,
  defined as follows: \\
$\transVar :=$
\begin{align*}
  \lambda \state \state'.\hspace{-1ex}
    \bigwedge_{\gen' \in \gens} 
    \state'(\gen') = sgn
    \hspace{-1ex}\left(
\sum_{\hspace{-3ex}\mathrlap{\{\gen \mid (\gen,\gen') \in \acts\}}} 
\state(\gen) \wVar(\gen) - %\quad~-\quad
\sum_{\hspace{-3ex}\mathrlap{\{ \gen \mid (\gen,\gen') \in \reps\}}}
\state(\gen) \wVar(\gen)
-
\thresh(\gen')
    \right)
\hspace{-1ex}\text{.}
\end{align*}  
% \end{itemize}
\end{defn}
%
The rest of the algorithm remains the same. 
%
\begin{example}(\exref{ex:oscilations} cont'd)\rm
The model of oscillation in \exref{ex:oscilations} can be modelled with a neg GRN without including the constant inputs to each gene.
%
The resulting parameter space would be simplified to:
 \begin{align*}
\grn_3 \models \prop_{3} & \hbox{ iff } (\weight_A>\thresh_B) \wedge (\weight_B>\thresh_C) \wedge (\weight_C>\thresh_A).
\end{align*} 
\end{example}

\subsection{Weights on edges}

%\ashu{Bio motivation for this variant}

So far, we assumed that each gene affects all other genes 
with the same weight.
%
Biologically, this corresponds to a situation when the mutations 
affect the coding sequence of the gene.  
%
In the `edge GRN' model variant, we allow that a gene affects other genes with
different weights.
%
This situation is arguably more realistic, since it is believed that the most 
common way for GRNs to evolve is through cis-regulatory mutations, i.e., 
mutations which affect the binding sites on the DNA, and not the coding sequence itself. % (which are in front of the coding sequence.
%, where the products of the  influencing genes bind to. 
In the modelling context, if a gene is influenced by more other genes, each of the influencing 
genes is assumed to have a different binding position, and hence, the binding strength, 
and consequently the affection of one gene to another does not depend on the other
weights affecting that same gene.

\begin{defn}[Edge GRN]\label{def:grnEdge} 
Edge GRN $\grn$ is a tuple \\ 
$(\gens,\acts,\reps,\weight, \thresh )$, where
\begin{itemize}
\item $\gens=\{\gene_1,\ldots,\gene_{\geneN}\}$ is a finite ordered set of genes,
\item $\acts \subseteq \gens \times \gens$ is the activation relation,
\item $\reps \subseteq \gens \times \gens$ is the repression relation,
\item $\weight \colon ( \acts \union \reps) \to \mathbb{R}_{\geq 0}$ is the weight
function, and
\item $\thresh \colon \gens \to \mathbb{R}_{\geq 0}$ is the threshold function.\footnote{see Appendix~\ref{sec:bio-mutation-model}
for the biological interpretation of weight and threshold functions}
\end{itemize}
\end{defn}
%
The difference from Def.~\ref{def:grn} is that weights are assigned 
to edges instead of genes. 
The weight $\weight(\gene,\gene')$ represents the strength of
influence of %activity of 
gene $\gene$ to 
%on activity of
 $\gene'$.
 %
For the edge GRN, the definition of the %states, runs, and 
semantics remain the same.
%
The definition of the transitions needs to be accordingly adjusted.

\begin{defn}[Transitions of an edge GRN]\label{def:grn-sem-e}
$\trans \colon \states(\grn)
\to \states(\grn)$ is a deterministic transition function defined by
\begin{align*}
\trans(\state):= \lambda\gen'. 
\left[
\quad
\sum_{\hspace{-8ex}\mathrlap{\{\gen \mid \state(\gen) \land (\gen,\gen') \in \acts\}}} 
\weight(\gen,\gen') \quad~-
\sum_{\hspace{-7ex}\mathrlap{\{ \gen \mid \state(\gen) \land (\gen,\gen') \in \reps\}}}
\weight(\gen,\gen')
 > \thresh(\gen')\right]\text{.}
\end{align*} 
\end{defn}

The change has to be incorporated also in the mutation model. 
%
Each interaction between two genes, say $\gene_i$ and $\gene_j$ is modelled by a nucleotide sequence of length $l_{ij}$.
%
The remaining model can then be inferred by the model of a single nucleotide mutation (\secref{sec:single}).

%
For a given topology, edge GRN model is a generalisation of 
our first model, in the sense that it can define a bigger range of GRNs.
%
The generalisation comes at the cost of larger parameter space and the robustness analysis becomes significantly more expensive
%
%More precisely, the dimensionality of the set of possible weights increases quadratically 
(while the weight function had 
dimension $d$ in the previous model, in the edge GRN, it has dimension $d^2$).
%


While edge GRN may exhibit mutational changes that are not possible in
GRN, this generality actually implies less efficient evolution -- a single mutation %change achieved in one generation
in the previous model affects the weight of many edges simulatneously which may be beneficial towards some phenotypes.



\paragraph{Efficient parameter search}
%
Alternatively, the analysis of edge GRN is amenable to a more efficient method than $\algGenCons$.
%
The value of a gene, say $\gene$, is affected by a set of genes from the GRN.
%
When the weights of these input genes change, the update of $\gene$ depends differently from the values of its affecters.
%
The parameters of these input weights can be split into regions, so that, whenever a set of parameters 
falls into a particular region, the update of gene $\gene$ depends in the same way on the values of the input genes.
%
In other words, each parameter region is assigned a boolean function over the 
input genes (e.g., in the neg GRN model, if one input gene $\gene'$ has a weight larger than all the others, then gene $\gene$
will always be updated to a previous value of $\gene'$).
%
In this way, the parameter search boils down to the enumeration of these regions and determining their boolean functions.
%
%Once the regions and corresponding boolean functions are found, the parameter regions which satisfy the property can be found by running the network for the set of all possible region values.
%
This idea can significantly improve the time of computing the constraints, because regions are determined for each gene locally, only by considering its input genes. 
%
Therefore for each gene, one can independently compute the space of
the weights on the input edges for which a gene manifests certain
boolean function~\cite{GRNSectorPaper2013}.
%
%
In other words, the problem is decomposed, and grows only linearly with the size of the GRN.
%
Since the number of boolean functions are finite, the space
of the weights is divided into finite regions. 
% 
%In edge GRN, the regions for every gene can be chosen independently, since the weights forming each region change independently.
%
Notice that this idea is not immediately applicable to the previous version of a GRN, since the regions of two different genes may depend on the same variable.
%if they are affected by some common genes.



As stated before, mutations in the edge GRN correspond to mutations in
the binding sites for a particular genes, while mutations in the first
model correspond to mutations in the coding sequences of the gene. 
%
In biology, is it thought that mutations in the coding sequences are
more likely to have adverse effects since they potentially affect all
the interactions the gene is involved in, an effect known as
pleiotropy. 
%
Our finding that GRNs can change several boolean function at a time,
while edge GRNs can only change one boolean function at a time,
reflects the pleiotropic nature of these networks.
%
Whether this impairs or aids evolution remains to be proved, but the
current formulation is a valuable tool to address this question.


%In the experimental section, we will compare the analysis of the above variants. 
%
In this paper, we do not advocate for any of the variants of the model.
%
Our goal is to illustrate that our method is applicable on such model variants.

 




%-------------------------------------------------------------------------------
%----------------- DO NOT ERASE THE TEXT BELOW THIS LINE -----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

